Secure Serverless Computing Using Dynamic Information Flow Control

The rise of serverless computing provides an opportunity to rethink cloud security. We present an approach for securing serverless systems using a novel form of dynamic information flow control (IFC). We show that in serverless applications, the termination channel found in most existing IFC systems can be arbitrarily amplified via multiple concurrent requests, necessitating a stronger termination-sensitive non-interference guarantee, which we achieve using a combination of static labeling of serverless processes and dynamic faceted labeling of persistent data. We describe our implementation of this approach on top of JavaScript for AWS Lambda and OpenWhisk serverless platforms, and present three realistic case studies showing that it can enforce important IFC security properties with low overhead.

==> background.tex <==
\section{Background on serverless computing}\label{sec:background}

Serverless computing emerged as part of the technological trend to
decouple application logic from resource management in the cloud.
In contrast to classic (\emph{monolithic}) software, applications
built with the cloud in mind, also known as \emph{cloud-native 
applications}, are designed as a collection of light-weight
\emph{microservices}~\cite{Newman-15}. 
The cloud platform automatically manages microservice placement, 
scheduling, and access to storage and other cloud services.
The cloud platform delivers elastic scalability by creating 
microservice instances based on demand. This requires application 
state to be decoupled from microservice instances and placed in a 
shared data store, allowing new instances to access the state.  

%Furthermore, since an instance can be destroyed at any time, any 
%state local to the instance must be disposable.

The serverless architecture formalizes this constraint by enforcing 
that every invocation of the service starts from a clean state.  In 
the serverless model, users express their applications as collections 
of functions.  A function can be written in any language, with many 
serverless applications containing functions in multiple languages.  
The function expects a certain runtime environment, defined by its 
developer, including, e.g., specific versions of the Python 
interpreter and libraries, but is agnostic of where this environment 
is instantiated: a physical machine, a virtual machine or a container.
Functions are triggered by several types of events, including user 
HTTP requests and calls from other functions.  Serverless functions 
are only expected to exchange data via shared data stores (databases, 
key value stores, network or local file systems) or by passing it as 
arguments to invocations\footnote{Current serverless platforms do not 
strictly enforce the clean state abstraction, allowing sequential  
invocations of a function hosted in the same container to share state, 
e.g., via global variables.  The \system sandbox prevents such sharing 
by resetting the JavaScript runtime to clean state on every 
invocation.}.

%The serverless architecture ephemarl nature of serverless function 
%invocations formalizes the state decoupeling constraint. As every 
%invocation potentially runs in a different environmentm and starts 
%from a clean state.  


%This design is meant to enable elastic scalability.  As we 
%demonstrate in the rest of this paper, it also has fundamental 
%implications for security.


Initially popularized by Amazon's AWS Lambda~\cite{AWSLambda}, 
serverless computing is rapidly gaining adoption by cloud providers 
and tenants due to its key benefits: elastic scalability, ease of 
deployment, and flexible pay-per-use pricing, with companies like  
Twitter~\cite{Eriksen-13}, Expedia~\cite{Expedia}, 
Coca-Cola~\cite{CocaCola}, iRobot~\cite{iRobot}, 
Reuters~\cite{Reuters}, and Nordstrom~\cite{HelloRetail} embracing 
serverless for their cloud backends.  Serverless is also finding new 
applications outside of the enterprise software domain, including 
real-time data processing~\cite{StreamAlert}, large-scale data 
analytics~\cite{Jonas-17}, and parallel computing~\cite{Fouladi-17}. 

In this work, we further strengthen the case for serverless computing 
by demonstrating that it enables practical information security in the 
cloud.




==> design-overview.tex <==
\section{Design Overview}

We are considering two alternative IFC algorithms.  The first one 
directly applies the standard progress-insensitive IFC from the 
literature in the serverless setting outlined in the previous section.  
The second one achieves progress sensitivity by introducing a faceted 
data store and assigning a maximal security label to each user 
request.

\subsection{Design 1}

Recall that a function can be triggered by (1) an external event, 
e.g., user request, (2) a data store update, or (3) another lambda.

\begin{itemize}
    \item We associate an effective security label $e$ with each 
        function activation.

    \item The effective label is initially set to the confidentiality 
        level of the source that triggered the activation (user's 
        security label in case (1) above, the security label of the 
        database update in case (2), or the effective security label 
        of the caller in case (3)).

    \item The effective label increases monotonically during execution 
        of the function as it reads confidential values from the data 
        store.

    \item The function can perform two types of I/O actions: (1) send 
        a message to an external output channel (e.g., the end-user 
        HTTP session) and (2) read or write the data store.  Both 
        actions are restricted by the following rules:

        \begin{itemize}
            \item The send operation is only allowed if the security 
                label of the output channel is greater than or equal 
                to $e$. Otherwise the send operation fails and the 
                function terminates.

            \item Consider a data store location that contains value v 
                with label $l$.  The activation can:
                \begin{itemize}
                    \item Read $v$. The effective label is set to the 
                        least upper bound of $e$ and $l$.

                    \item Write $v$ if $e \leq l$. The effective label 
                        does not change. The store location inherits 
                        label $e$.  The write operation fails 
                        otherwise, terminating execution of the 
                        function (the no-sensitive-upgrade rule).
                \end{itemize}
        \end{itemize}
\end{itemize}

One problem with this design is that it leaks information whenever a 
send or write operation fails.  In the serverless setting, where a 
single request can spawn any number of concurrent functions, unbounded 
amount of information can leak in this way through a single request.

\subsection{Design 2}

We therefore consider an alternative design that attempts to eliminate 
this channel. The key idea is to statically assign a maximal security 
label to each user request and modify the data store behavior to 
conceal the presence of any data with higher security labels.

\begin{itemize}
    \item We associate two security labels with an activation: an 
        effective label $e$ and the maximal label $m$.

    \item As before, the effective label is initially set to the 
        confidentiality level of the source that triggered the 
        activation.

    \item The effective label increases monotonically during execution 
        of the function as it reads confidential values from the data 
        store.

    \item Our secure runtime ensures that the effective label may not 
        exceed the maximal label ($e \leq m$).

    \item The maximal label is assigned by the secure runtime when the 
        function is being triggered by the user or by a data store 
        update and is inherited from the caller when the function is 
        invoked by another function. It must be greater than or equal 
        to the initial value of the effective label.  Importantly, 
        when the label is assigned by the runtime, its value must not 
        depend on any secret data above the initial effective label 
        (i.e., the confidentiality level of $m$ is $\leq e$).

    \item The function can perform two types of I/O actions: (1) send 
        a message to an external output channel (e.g., the end-user 
        HTTP session) and (2) read or write the data store.  Both 
        actions are restricted by the following rules, which 
        (hopefully) enforce confidentiality:

        \begin{itemize}
            \item The security label of the output channel must be 
                greater than or equal to the maximal security label of 
                the activation.  Note that using the maximal security 
                label, rather than the effective one, is essential to 
                preventing information leaks.

            \item Consider an activation with effective and maximal 
                labels $e$ and $m$ respectively and a data store 
                location that contains value $v$ with label $l$.  Our 
                secure data store semantics \emph{conceals} the 
                existence of any data whose confidentiality level is 
                higher than or incomparable to $m$ ($l \nleq m$).  
                
                We first consider the simple case where security 
                labels form a total order. The corresponding data 
                store semantics is given in Table~\ref{ta:ifc-total}, 
                with the write operation specified as 
                $\semruletxt{\tuple{e,l}}{w}{\tuple{e',l'}}$, and the 
                read operation specified as 
                $\semruletxt{\tuple{e,l}}{r}{\tuple{e',l'}, v'}$, 
                where $e$ and $l$ are the effective security label of 
                the function and the security label of the data store 
                location before the operation; $e'$ and $l'$ are the 
                new security labels after the operation, $m$ is the 
                maximal security label of the function, and $v'$ is 
                the value returned by the read operation, or the 
                special $empty$ value.

                Intuitively, the write operation overwrites the data 
                store location with the new value and security label, 
                unless the data store contains a less secret label, in 
                which case the write fails (enforcing the the 
                no-sensitive-upgrade policy).  A read returns the 
                value in the data store, tainting the function with 
                its label, unless the data store location has 
                confidentiality label $l>m$, in which case the $empty$ 
                value is returned.  
        
            \item We now consider the general case where security 
                labels form a lattice.  Table~\ref{ta:ifc-partial} 
                gives the operational semantics in this case.  

                We introduce faceted data store, where each location 
                contains a set of values with incomparable security 
                labels.  The write behavior depends on whether there 
                exists a facet with a comparable label in the data 
                store.  If a comparable facet exists, the write will 
                either overwrite its value or fail if the data store 
                label is lower than $e$ (no sensitive upgrade).  
                Otherwise, a new facet is created.  

                The read operation returns $empty$ if no facet whose 
                label $l$ is $\leq m$ exists in the data store; 
                alternatively is a unique such facet exists, it 
                returns the value in that facet; finally, if more than 
                one such face exists in the data store, an error is 
                returned.
        \end{itemize}
\end{itemize}


==> model.tex <==
\section{Model} % (fold)
\label{sec:model}

In this section we present a model for describing information flow in a transactional system.

\subsection{Computational Model} % (fold)
\label{sub:computational_model}
We begin by describing the non-IFC computational model.

Our model consists of a set of memory locations $M=\{m_1,\dots,m_n\}$, a memory access function $r: M \rightarrow D$, where $D$ is the domain of data in our system, and a set of computations $\mathcal{F} = \{f_1,\ldots,f_k\}$ where each copmutation $f_i$ is a function from a vector of data elements to a single data element $f_i:\overline{D} \rightarrow D$.

We define a \emph{transaction} operation that applies a given computation to the values stored in a vector of memory locations, and stores the result of the computation in another memory location. \TODO{Semantics for the transaction operation.}

% subsection computational_model (end)


% section model (end)

==> semantics.tex <==
%\section{Semantics}

%Tables~\ref{ta:ifc-total} and~\ref{ta:ifc-partial} summarize the 
%proposed operational semantics for totally and parially ordered
%security labels respectively.

\begin{table*}
\[
\begin{array}{lclr}
\hline\hline
\semrule{\tuple{e,empty}}{w}{\tuple{e,e}}{\mbox{write to an empty cell in the data store}}\\
\hline
\semrule{\tuple{e,l}}{w}{\case{\mbox{error}}{\mbox{if} ~ e > l}{\tuple{e,e}}{\mbox{otherwise}}} {\mbox{write to a cell in the data store}}\\
\hline
\semrule{\tuple{e,empty}}{r}{\tuple{e,empty}, empty}{\mbox{read an empty cell in the data store}}\\
\hline
\semrule{\tuple{e,l}}{r}{\case{\tuple{max(e,l),l}, v}{\mbox{if} ~ m \geq l}{\tuple{e,l}, empty}{\mbox{otherwise}}} {\mbox{read a cell in the data store}}\\
\hline\hline
\end{array}
\]
\caption{\label{ta:ifc-total}%
Small-step operational semantics for enforcing IFC with a total order over the security labels. $m$ is a paramater of the program execution s.t. m is the maximal security label allowed for the execution.}
\end{table*}

\begin{table*}
\[
\begin{array}{lclr}
\hline\hline
\semrule{\tuple{e,\emptyset}}{w(v)}{\tuple{e,\{\tuple{v,e}\}}}{\mbox{write to an empty cell in the data store}}\\
\hline
\semrule{\tuple{e,S}}
        {w(v)}
        {\case{\mbox{error}}
              {\exists \tuple{v',l'} \in S. ~ l' < e}
              {\tuple{e,(S \setminus \{\tuple{v',l'} | l' \geq e \}) \cup \{\tuple{v,e}\}}}
              {\mbox{otherwise}}}
        {\mbox{write to a cell in the data store}}\\
\hline
\semrule{\tuple{e,\emptyset}} {r} {\tuple{e,\emptyset}, empty} {\mbox{read an empty cell in the data store}}\\
\hline
\multicolumn{4} {l} {\mbox{let}~ S\!\downarrow_m = \{\tuple{v,l}\in S | l \leq m\} }\\
\semrule{\tuple{e,S}}
        {r}
        {\casethree{\tuple{e,S}, empty} {|S\!\downarrow_m| = 0}
                   {\tuple{max(e,l), S}, v} {|S\!\downarrow_m| = 1}
                   {\mbox{error}}{|S\!\downarrow_m| > 1}}
        {\mbox{read a cell in the data store}}\\
\hline\hline
\end{array}
\]
\caption{\label{ta:ifc-partial}%
Small-step operational semantics for enforcing IFC with a partial order over the security labels. $m$ is a paramater of the program execution s.t. m is the maximal security label allowed for the execution.}
\end{table*}

\section{Discussion}

While faceting prevents leaking of information through termination, it 
also changes the semantics of the data store expected by the 
application.  However this should not occur during normal operation.  
Creation of multiple facets indicates an attempted security violation 
and is signaled to the administrator. While the issue is being 
resolved, faceting continues to enforce confidentiality.

%We employ two techniques to enforce confidentiality at the data-store
%level: (1) faceting and (2) the no-sensitive-upgrade (NSU) rule.  The former
%restricts information flow by presenting different views of the store
%to different observers.  We use it to isolate writes by incomparable 
%users.  The latter prevents the flow of information down the lattice by
%blocking high writes to low locations.  Both mechanisms preserve
%termination sensitivity.
%\TODO{Does NSU preserve termination sensitivity?
%I thought it would leak half a bit by continuing execution in some
%cases while raising an error in other cases. --Tommy}
%NSU reduces faceting (which can be seen as a
%form of store corruption that requires manual intervention) by
%sacrificing transparency.  Without NSU, we would need to introduce
%facets for each label, not just incomparable ones.

\section{Properties of the Semantics}

Below we state some properties of our proposed scheme which need to be verified w.r.t.
a formal semantics of executions.

\begin{conj}
Our semantics enforces termination-sensitive noninterference, i.e., whenever there exists
a way to violate the information flow requirement, it enforces noninterference by either yielding an error (the no-sensitive-upgrade case)
or faceting the data store (the incomparable writes case).
\end{conj}

\begin{conj}
Our semantics can be easily implemented for Javascript programs using
any key value DB with very low runtime overhead.
\end{conj}

\begin{conj}
Our semantics can identify interesting bugs in real applications.
\end{conj}

\begin{conj}
Our semantics is not transparent, i.e., there exist correct programs for which our semantics
will yield error.
\end{conj}

\begin{conj}
In practical serverless applications, the no-sensitive-upgrade semantics is preferable to transparency
as it avoids data store corruption.
\end{conj}

\begin{conj}
Correct programs which are rejected by our semantics can be modified to work with our IFC model with modest implementation effort.
\end{conj}

%\section{Partial Order}

